Hierarchical Clustering Can Jointly Satisfy Richness, Consistency, and Scale Invariance

Despite its ubiquity, clustering lacks a universally accepted definition of what is a cluster. Kleinberg's Impossibility Theorem formalizes this difficulty by showing that no flat clustering method can simultaneously satisfy three natural axioms: scale invariance, richness, and consistency. In this paper, we ask whether this impossibility persists when the output is a hierarchy rather than a single partition. We show that, in contrast to the flat clustering setting, the hierarchical analog of these axioms are jointly satisfiable. In fact, there exist uncountably many hierarchical clustering methods satisfying these axioms, which we call admissible. We explicitly construct several admissible methods, including methods based on well-separated clusters and a non-binary version of single linkage. For certain pairs of admissible methods, the hierarchy produced by one always refines that produced by the other. This refinement relation defines a partial order on the class of admissible methods. This partially ordered set has no greatest element and contains uncountably many pairwise incompatible maximal elements, revealing substantial diversity among admissible methods. Nevertheless, this diversity is constrained: every admissible method contains a hierarchy of sufficiently well-separated clusters, and every finite collection of admissible methods shares such a nontrivial common backbone.

==> header.tex <==
% \usepackage{bbm}
% \usepackage{dsfont}
% \usepackage{epsf}
% \usepackage{fancyhdr}
% \usepackage{graphics}
% \usepackage{graphicx}
% \usepackage{psfrag}
% \usepackage[dvipsnames]{xcolor}

% \usepackage{amsthm}
% \usepackage{amsfonts}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{bbm}

% \usepackage[utf8]{inputenc}
% \usepackage[colorlinks=true, allcolors=blue]{hyperref}
% % \usepackage[authoryear]{natbib}
% % \usepackage{appendix}

\usepackage{tikz}
\usetikzlibrary{arrows.meta,positioning, fit, backgrounds, calc}
\usepackage{mathtools}
\usepackage{mathabx}
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{subcaption}
% \newsavebox{\bigimage}
\usepackage{multirow}
% \usepackage{float}
% \usepackage[nodisplayskipstretch]{setspace} 
% % \usepackage[capitalise,noabbrev,nameinlink]{cleveref}
% %\usepackage{bm}
% \usepackage{dsfont}
% \usepackage{xspace}
% \usepackage{pifont}%

% \usepackage{microtype}
\usepackage{booktabs} % for professional tables

\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\RequirePackage{forloop}
% \RequirePackage{url}



% \newtheorem{claim}{Claim}
% \newtheorem{fact}{Fact}
\newtheorem{observation}{Observation}
% \newtheorem{setting}{Setting}
% \newtheorem{example}{Example}
% \newtheorem{property}{Property}
% \newtheorem{condition}{Condition}
% \newtheorem{violation}{Violation}



% \newcommand{\independent}{\perp\mkern-9.5mu\perp}
% \newcommand{\notindependent}{\centernot{\independent}}


% % ICML
% % if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % THEOREMS
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{axiom}{Axiom}[section]
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}

\newtheorem{namedlist}{List}


\newcommand{\updated}[1]{\textcolor{red}{#1}}
\newenvironment{oldtext}
{\par \small \color{gray}
{\bf Old text. Either deprecated or not relevant anymore, to be deleted later. %Please remove me when you have checked that the new text is okay.
}
}
{\par}
\newenvironment{newtext}
{\par \small \color{blue}
{\bf New text.}
}
{\par}

% AUTHOR COMMENTS
\newcommand{\MD}[1]{\textcolor{violet}{MD: #1} }
\newcommand{\MG}[1]{\textcolor{teal}{MG: #1} }
\newcommand{\MDnote}[1]{\textcolor{violet}{\small {\bf MD}: #1}}
\newcommand{\DK}[1]{\textcolor{magenta}{D: #1} }
\newcommand{\TODO}[1]{\textcolor{purple}{TODO: #1} }
\newcommand{\PT}[1]{\textcolor{orange}{PT: #1} }

